UniMem: Towards a Unified View of Long-Context Large Language Models

Long-context processing is a critical ability that constrains the applicability of large language models (LLMs). Although there exist various methods devoted to enhancing the long-context processing ability of LLMs, they are developed in an isolated manner and lack systematic analysis and integration of their strengths, hindering further developments. In this paper, we introduce UniMem, a Unified framework that reformulates existing long-context methods from the view of Memory augmentation of LLMs. Distinguished by its four core dimensions-Memory Management, Memory Writing, Memory Reading, and Memory Injection, UniMem empowers researchers to conduct systematic exploration of long-context methods. We re-formulate 16 existing methods based on UniMem and analyze four representative methods: Transformer-XL, Memorizing Transformer, RMT, and Longformer into equivalent UniMem forms to reveal their design principles and strengths. Based on these analyses, we propose UniMix, an innovative approach that integrates the strengths of these algorithms. Experimental results show that UniMix achieves superior performance in handling long contexts with significantly lower perplexity than baselines.

==> Figures/Fig-Exp-memoryLayerAllocation.tex <==
\begin{figure*}[!t]
    \vspace{-1.0em}
    \centering
    \subfigure[Impact of Memory Layer Distribution.]{
        %\centering
        \begin{minipage}[c][][c]{0.35\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/tinyllama_mix_memory_layer_distribution.png}
            %\vspace{0.1pt}
            % \caption{aaa}
        \end{minipage}
        % \caption{}
        % \label{fig:ppl-layer-distribution}
        \label{fig:ppl-mix-memory—layer-distribution}
    }
    \hspace{2cm}  % 添加 1 厘米的水平间距
    \subfigure[Impact of Memory Layer Position.]{
        %\centering
        \begin{minipage}[c][][c]{0.42\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/tinyllama_mix_github+pg19_singlelayer1.png}
            %\vspace{0.1pt}
        \end{minipage}
        % \vfill
        % \caption[b]{Memorizing Transformer}
        \label{fig:ppl-mix-singlelayer}
    }
    \setlength{\abovecaptionskip}{1pt} % 调整图与标题之间的垂直间距
    \caption{The Effect of Memory Layer Alterations on UniMix's Perplexity}
    \label{fig:memoryLayerAllocation}
    \vspace{-1.0em}
\end{figure*}

==> Figures/Fig-Exp-multiDimension.tex <==
\begin{figure}[t]
    \centering
    \subfigure[Memory Layer Distribution]{
        \centering
        % \begin{subfigure}[t]{0.46\textwidth}
        \includegraphics[width=0.20\textwidth]{Figures/RawFiles/Topk2.png}
        \caption{Impact of \emph{topk} on perplexity for MemTrans and \textbf{Mix methods}.}
        \label{fig:ppl-topk}
    }
    \hfill  % 添加一些水平间距
    \subfigure[Memory Layer Position Exploration]{
        \centering
        % \begin{subfigure}[t]{0.46\textwidth}
        \includegraphics[width=0.20\textwidth]{Figures/RawFiles/Window.png}
        \caption{Impact of \emph{window length} on perplexity for Trans-XL and \textbf{Mix} methods.}
        \label{fig:ppl-window}
    }
    \hfill  % 添加一些水平间距
    \caption{Perplexity of Mix mode with Memory Layer Allocation Change.}
    \label{fig:memoryLayerAllocation}
\end{figure}

==> Figures/Fig-Exp-window+topk-change.tex <==
\begin{figure}[!t]
    \centering
    \subfigure{
    \begin{minipage}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/RawFiles/Topk2.png}
        \caption{Impact of \textit{Topk} on perplexity for MemTrans and \textbf{UniMix}.}
        \label{fig:ppl-topk}
    \end{minipage}
    }
    \hspace{1cm}  % 添加 1 厘米的水平间距
    \subfigure{
    \begin{minipage}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/RawFiles/Window.png}
        \caption{Impact of \textit{window length} on perplexity for Trans-XL and \textbf{UniMix}.}
        \label{fig:ppl-window}
    \end{minipage}
    }
\end{figure}

==> Figures/Fig.Exp-ExistingMethod.tex <==
% \begin{figure}[t]
%     \centering
%     % \begin{subfigure}[t]{0.46\textwidth}
%     \includegraphics[width=0.455\textwidth]{Figures/RawFiles/exp-existMethod.png}
%     \caption{Perplexity of different methods in Unimem Veiw.}
% \end{figure}

\begin{figure*}[t]
    \centering
    \subfigure[TinyLlama on the Github]{
        \centering
        \begin{minipage}[c][][c]{0.23\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/exp-existMethod.png}
            % \caption{aaa}
        \end{minipage}
        % \caption{}
        \label{fig:ppl-github}
    }
    \hfill  % 添加一些水平间距
    \subfigure[TinyLlama on the PG19]{
        \centering
        \begin{minipage}[c][][c]{0.23\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/exp-existMethod.png}
        \end{minipage}
        % \vfill
        % \caption[b]{Memorizing Transformer}
        \label{fig:ppl-pg19}
    }
    \hfill  % 添加一些水平间距
    \subfigure[Llama2 on the Github]{
        \centering
        \begin{minipage}[c][][c]{0.23\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/7b_existingMethods.png}
        \end{minipage}
        % \vfill
        % \caption{RMT}
        \label{fig:ppl-7b}
    }
    % \hfill  % 添加一些水平间距
    \subfigure[TinyLlama on the Github]{
        \centering
        \begin{minipage}[c][][c]{0.23\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/PI.png}
        \end{minipage}
        % \vfill
        % \caption{Longformer}
        \label{fig:ppl-pi}
    }
    \caption{Perplexity of different methods in Unimem Veiw.}
\end{figure*}

==> Figures/Fig.Exp-Llama2-Mix-SingleLayer.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/llama2_mix_singlelayer.png}
    \caption{Perplexity of Single Layer on \textbf{UniMix}(Llama2-7B)}
    \label{fig:ppl-mix-singlelayer-llama2}
\end{figure}

==> Figures/Fig.Exp-MaxLength.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/MaxLength.png}
    \caption{Max length of Vanilla and Unimem mix.}
\end{figure}

==> Figures/Fig.Exp-PI.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/PI.png}
    \caption{Progression of perplexity reduction between Position Interpolation(PI) and the \textbf{Mix} method across equivalent training tokens.}
    \label{fig:ppl-only-PI}
\end{figure}

==> Figures/Fig.Exp-SingleDimension.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/Window.png}
    \caption{Perplexity when varifying window length hyperparameter}
\end{figure}

==> Figures/Fig.Exp-Tinyllama-Longformer-0-10+16.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/tinyllama_longformer_0-10+16.png}
    \caption{Perplexity of Layer(1-11) and Layer(16) on Longformer}
    \label{fig:ppl-longformer-(0-10)&16}
\end{figure}

==> Figures/Fig.Exp-Tinyllama-Memtrans-0-10+16.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/tinyllama_memtrans_0-10+16.png}
    \caption{Perplexity of Layer(1-11) and Layer(16) on Memtrans}
    \label{fig:ppl-memtrans-(0-10)&16}
\end{figure}

==> Figures/Fig.Exp-Tinyllama-Memtrans-SingleLayer.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/tinyllama_memtrans_singlelayer.png}
    \caption{Perplexity of Single Layer on Memtrans(TinyLlama)}
    \label{fig:ppl-memtrans-singlelayer}
\end{figure}

==> Figures/Fig.Exp-Tinyllama-Mix-0-10+11-21.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/tinyllama_mix_0-10+11-21.png}
    \caption{Perplexity of Layer(0-10) and Layer(11-21) on Mix}
    \label{fig:ppl-mix-(0-10)&(11-21)}
\end{figure}

==> Figures/Fig.Exp-Tinyllama-Mix-0-6+7-13+14-20.tex <==
\begin{figure}[H]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.4\textwidth]{Figures/RawFiles/tinyllama_mix_0-6+7-13+14-20.png}
    \caption{Perplexity of Layer(1-7), Layer(8-14) and Layer(15-21) on Mix}
    \label{fig:ppl-mix-(0-6)&(7-13)&(14-20)}
\end{figure}

==> Figures/Fig.Exp-Tinyllama-Mix-SingleLayer-PG19.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/tinyllama_pg19_mix_singlelayer.png}
    \caption{Perplexity of Single Layer on Mix(PG19, TinyLlama)}
    \label{fig:ppl-mix-singlelayer-pg19}
\end{figure}

==> Figures/Fig.Exp-Tinyllama-Mix-SingleLayer.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/tinyllama_mix_singlelayer.png}
    \caption{Perplexity of Single Layer on Mix(TinyLlama)}
    \label{fig:ppl-mix-singlelayer}
\end{figure}

==> Figures/Fig.Exp-Tinyllama-Trans_xl-0-10+16.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/tinyllama_xl_0-10+16.png}
    \caption{Perplexity of Layer(1-11) and Layer(16) on TransXL}
    \label{fig:ppl-xl-(0-10)&16}
\end{figure}

==> Figures/Fig.Exp-VarifyDim.tex <==
\begin{figure*}[t]
    \centering
    \subfigure[Secondary Memory Size]{
        \centering
        \begin{minipage}[c][][c]{0.31\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/rmt_size.png}
            % \caption{aaa}
        \end{minipage}
        % \caption{}
        \label{fig:varify-rmt_size}
    }
    \hfill  % 添加一些水平间距
    \subfigure[Topk]{
        \centering
        \begin{minipage}[c][][c]{0.31\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/topk.png}
        \end{minipage}
        % \vfill
        % \caption[b]{Memorizing Transformer}
        \label{fig:varify-topk}
    }
    \hfill  % 添加一些水平间距
    \subfigure[Sliding Window Length]{
        \centering
        \begin{minipage}[c][][c]{0.31\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/windows.png}
        \end{minipage}
        % \vfill
        % \caption{RMT}
        \label{fig:varify-windows}
    }
    \caption{Perplexity when varifying different Dimensions}
\end{figure*}

==> Figures/Fig.Exp-VarifyDimDelta.tex <==
\begin{figure*}[t]
    \centering
    \subfigure[Secondary Memory Size]{
        \centering
        \begin{minipage}[c][][c]{0.49\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/topk_delta.png}
            % \caption{aaa}
        \end{minipage}
        % \caption{}
        \label{fig:varify-delta_topk}
    }
    \hfill  % 添加一些水平间距
    \subfigure[Topk]{
        \centering
        \begin{minipage}[c][][c]{0.49\linewidth}
            \includegraphics[width=\textwidth]{Figures/RawFiles/windows_delta.png}
        \end{minipage}
        % \vfill
        % \caption[b]{Memorizing Transformer}
        \label{fig:varify-delta_windows}
    }
   
    \caption{Perplexity delta in Exsiting Methods and in Mix}
\end{figure*}

==> Figures/Fig.Exp-window_change.tex <==
\begin{figure}[!t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \setlength{\belowcaptionskip}{-1pt}
    \includegraphics[width=0.35\textwidth]{Figures/RawFiles/Window.png}
     \setlength{\abovecaptionskip}{-1pt}
    \caption{Impact of \textit{window length} on perplexity for Transformer-XL and UniMix.}
    \label{fig:ppl-window}
    \vspace{-1.0em}
\end{figure}

==> Figures/Fig.Overview.tex <==
\begin{figure}[t]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.455\textwidth]{Figures/RawFiles/Unimem Overview.png}
    \caption{Unimem Overview.}
\end{figure}

==> Figures/Fig.rmt_change.tex <==
\begin{figure}[H]
    \centering
    % \begin{subfigure}[t]{0.46\textwidth}
    \includegraphics[width=0.3\textwidth]{Figures/RawFiles/rmt_size.png}
    \caption{Impact of \emph{Memory Tokens} on perplexity for \textbf{Mix methods}.}
    \label{fig:ppl-rmt}
\end{figure}

==> Figures/Fig.unimem-view2.tex <==
\begin{figure*}[t]
    \centering
    % \begin{subfigure}[t]{0.43\textwidth}
    \subfigure[RMT]{
        \centering
        \includegraphics[width=0.43\textwidth]{Figures/RawFiles/uni-rmt.pdf}
        % \caption{RMT}
        \label{fig:uni-rmt}
    % \end{subfigure}
    }
    \hfill  % 添加一些水平间距
    % \begin{subfigure}[t]{0.52\textwidth}
    \subfigure[Longformer]{
        \centering
        \includegraphics[width=0.52\textwidth]{Figures/RawFiles/uni-longformer.pdf}
        % \caption{}
        \label{fig:uni-longformer}
    % \end{subfigure}
    }
    \caption{Illustration of Recurrent Memory Transformers (RMT) and Longformer in the context of the UniMem framework. The yellow circles mark segments processed in earlier steps, while the blue circles denote the segment currently undergoing processing. The RMT employs a specialized memory token to capture information from one prior segment, which, after \textcolor{
    brown}{model forwarding}, is stored in the \textcolor{gray}{memory cache}. This information is then accessible across all layers during the processing of the current segment. The Longformer, on the other hand, stores hidden states from multiple previous segments directly into the \textcolor{gray}{memory cache}. It retrieves this information using a mechanism known as \textcolor{pink-line}{global attention} and \textcolor{green-line}{sliding window attention}, which are based on the relative positioning of tokens.}
    \label{fig:uni-view2}
\end{figure*}

==> Tables/Draft_dimension_v2.tex <==
\begin{table}[t]
    \vspace{-1.0em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}*{Method} & \multicolumn{2}{c}{Memory cache management} & \multirow{2}*{Memory Write} & \multirow{2}*{Memory Read} & \multirow{2}*{Memory Layer Allocation} & \multirow{2}*{Memory Gradient Propagation} \\
       
          &      Memory scale  & Memory cache update        & &  \\
        \midrule
      RMT\cite{rmt}       &         single chunk  &   FIFO   &      model forward  &                      All                  & Each layer  & BPTT  \\
AutoCompressor\cite{chevalier2023adapting}  &    multi chunk  &   undefined        &      model forward  &                      All                  & Each layer   & BPTT  \\
\\
Longformer\cite{longformer}      &    multi chunk  &   clear all   &            direct        &                     Position              & Each layer   & BPTT  \\
Bigbird\cite{bigbird}         &    multi chunk  &   clear all   &             direct         &                     Position              & Each layer   & BPTT  \\
LongNet\cite{ding2023longnet}        &     multi chunk  &   clear all   &            direct          &                     Position              & Each layer   & BPTT \\
Transformer-XL\cite{transformer-xl}  &   single chunk  &   FIFO       &           direct            &                     Position              & Each layer   & Stop \\
StreamingLLM\cite{xiao2023efficient}    &    multi chunk   &   FIFO        &           direct           &                    Position              & Each layer   & BPTT  \\
\\
MemTrans\cite{memorizing}  &  multi chunk &  FIFO    &          direct            &                  Similarity            & Certain layers  & Stop \\
FoT\cite{tworkowski2023focused}  &  multi chunk &  FIFO    &          direct            &                  Similarity            & Certain layers  & Crossbatch \\
Unilimiformer\cite{bertsch2023unlimiformer}          &  multi chunk &  undefined    &          direct            &                  Similarity            & Each layer  & Stop   \\
Routing\cite{roy2021efficient}     &  multi chunk &  clear all    &         direct           &               Similarity            & Each layer & BPTT  \\
Reformer\cite{kitaev2020reformer}               &  multi chunk &  clear all    &       direct            &                 Similarity            & Each layer & BPTT   \\
\\
Poolingformer\cite{zhang2021poolingformer}   & multi chunk &         clear all      &     pooling+direct       &               Position          & Each layer & BPTT \\
LongT5\cite{guo2021longt5}     & multi chunk &         clear all      &       pooling+direct       &                  Position          & Each layer & BPTT  \\

\\
% RetNet\cite{bulatov2022recurrent}       &         single chunk  &   FIFO   &      model forward  &                      All                  & Each layer  & BPTT \\
KNN-LM\cite{khandelwal2019generalization}   & Corpus &         /      &     direct       &               Similarity          & Certain layer & / \\
TRIME\cite{zhong2022training}     & / &         clear all      &       direct       &                  Similarity          & Certain layer & Contrastive loss  \\

    \bottomrule
    \end{tabular}
    }
    \caption{Long text extension methods decomposed along the defined design dimensions}
    \vspace{-1.0em}
\end{table}

==> Tables/Draft_unimem_dimension.tex <==
\begin{table}[h]
    \vspace{-1.0em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}*{Method} & \multicolumn{2}{c}{Memory cache management} & \multirow{2}*{Memory Write} & \multirow{2}*{Memory Read} & \multicolumn{2}{c}{Detail\fjj{Traing trick / Memory utilize}} \\
       
          &      Memory scale  & Memory cache udpate        &    &     & Memory layer & BPTT rollout \\
        \midrule
      RMT       &         single chunk  &   clear all   &      model forward  &                      All                  & Each layer  & yes  \\
AutoCompressor  &    multi chunk  &   \fjj{clear all}        &      model forward  &                      All                  & Each layer   & no  \\
\\
Longformer      &    multi chunk  &   clear all   &            direct        &                     Position              & Each layer   & yes  \\
Bigbird         &    multi chunk  &   clear all   &             direct         &                     Position              & Each layer   & yes  \\
LongNet        &     multi chunk  &   clear all   &            direct          &                     Position              & Each layer   & yes \\
Transformer-XL  &   single chunk  &   FIFO       &           direct            &                     Position              & Each layer   & no \\
StreamingLLM    &    multi chunk   &   FIFO        &           direct           &                    Position              & Each layer   & \fjj{yes}  \\
\\
Memorizing  &  multi chunk &  FIFO    &          direct            &                  Similarity            & Certain layers  & no \\
\fjj{FoT}  &  \fjj{single/multi chunk} &  FIFO    &          direct            &                  Similarity            & Certain layers  & \fjj{yes} \\
Unilimiformer          &  multi chunk &  \fjj{clear all}    &          direct            &                  Similarity            & Each layer  & no   \\
Routing     &  multi chunk &  clear all    &         direct           &               Similarity            & Each layer & yes  \\
Reformer               &  multi chunk &  clear all    &       direct            &                 Similarity            & Each layer & yes   \\
\\
Poolingformer   & multi chunk &         clear all      &     pooling+direct       &               Position          & Each layer & yes \\
LongT5     & multi chunk &         clear all      &       pooling+direct       &                  Position          & Each layer & yes  \\

\\
\fjj{KNN-LM}   & \fjj{Corpus} &         \fjj{/}      &     direct       &               Similarity          & Certain layer & \fjj{/} \\
\fjj{TRIME}     & \fjj{single/multi chunk} &         clear all      &       direct       &                  Similarity          & Certain layer & no  \\

    \bottomrule
    \end{tabular}
    }
    \caption{Long text extension methods decomposed along the defined design dimensions \fjj{Training or Inference?}}
    \vspace{-1.0em}
\end{table}

==> Tables/Tab.unimem-formulation.tex <==
\begin{table}[t]
\vspace{-1.0em}
% \caption{UniMem. \label{tab:unimem}}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l}
\toprule
%% ************************************
\textbf{Stage} & \textbf{Methods} &  \textbf{Formulations} 
\\ \hline
\multirow{5}{*}{Memory Retrieval} & Transformer-XL & $\mathbf{K}_{m}^{n}/\mathbf{V}_{m}^{n} \leftarrow \mathbf{K}_{\tau\text{-}1}^{n}/\mathbf{V}_{\tau\text{-}1}^{n}$ 
\\ 
& Memorizing Transformer & $\mathbf{K}_{m}^{n}/\mathbf{V}_{m}^{n} \leftarrow \mathop{\text{Top K}^\text{KNN}} (\mathbf{q}_{\tau}^n \cdot \mathbf{k}_{m}^n)$ ;\text{  } $\mathbf{k}_{m}^n/\mathbf{v}_{m}^n \in \mathbf{K}_{1:\tau\text{-}1}^{n} /\mathbf{\mathbf{V}}_{1:\tau\text{-}1}^{n}$
\\ 
& RMT & $\mathbf{K}_{m}^{n}/\mathbf{V}_{m}^{n} \leftarrow \mathbf{M}_{\tau}^{n-1}(\mathbf{W}_{q}^{n})^T/\mathbf{M}_{\tau}^{n-1}(\mathbf{W}_{v}^{n})^T$ ;\text{  } $\mathbf{M}_{\tau}^{0} = \overline{\mathbf{M}}_{\tau-1}^{N}$
\\ 
& Longformer & $\mathbf{K}_{m}^{n}/\mathbf{V}_{m}^{n} \leftarrow [\mathbf{K}_{\tau\text{-}1}^{n} \circ \mathbf{K}_{g}^{n}]/[\mathbf{V}_{\tau\text{-}1}^{n} \circ \mathbf{V}_{g}^{n}]$ 
\\
& StreamingLLM & $\mathbf{K}_{m}^{n}/\mathbf{V}_{m}^{n} \leftarrow [\mathbf{K}_{\tau\text{-}1}^{n} \circ \mathbf{K}_{g}^{n}]/[\mathbf{V}_{\tau\text{-}1}^{n} \circ \mathbf{V}_{g}^{n}]$ 
\\
& BigBird & $\mathbf{K}_{m}^{n}/\mathbf{V}_{m}^{n} \leftarrow [\mathbf{K}_{\tau\text{-}1}^{n}  \circ \mathbf{K}_{g}^{n} \circ \mathbf{K}_{r}^{n}]/[\mathbf{V}_{\tau\text{-}1}^{n} \circ \mathbf{V}_{g}^{n} \circ \mathbf{V}_{r}^{n}]$ 
\\ \hline
\multirow{5}{*}{Memory Update} & Transformer-XL & $\mathbf{K}_{\tau\text{-}1}^{n}/\mathbf{V}_{\tau\text{-}1}^{n} \leftarrow \mathbf{K}_{\tau}^{n}/\mathbf{V}_{\tau}^{n}$
\\ 
& Memorizing Transformer & $\mathbf{K}_{1:\tau\text{-}1}^{n}/\mathbf{\mathbf{V}}_{1:\tau\text{-}1}^{n} \leftarrow \mathbf{K}_{1:\tau}^{n} /\mathbf{V}_{1:\tau}^{n}$
\\
& RMT & $\overline{\mathbf{M}}_{\tau-1}^{N} \leftarrow \overline{\mathbf{M}}_{\tau}^{N}$
\\
& Longformer & $\mathbf{K}_{\tau\text{-}1}^{n}/\mathbf{V}_{\tau\text{-}1}^{n} \leftarrow \mathbf{K}_{\tau}^{n}/\mathbf{V}_{\tau}^{n}$
\\ 
& StreamingLLM & $\mathbf{K}_{\tau\text{-}1}^{n}/\mathbf{V}_{\tau\text{-}1}^{n} \leftarrow \mathbf{K}_{\tau}^{n}/\mathbf{V}_{\tau}^{n}$
\\ 
& Big Bird & $\mathbf{K}_{\tau\text{-}1}^{n}/\mathbf{V}_{\tau\text{-}1}^{n} \leftarrow \mathbf{K}_{\tau}^{n}/\mathbf{V}_{\tau}^{n}$
\\
% \\ \hline
% \multirow{5}{*}{BPTT Step} & Transformer-XL & $1$ step
% \\
% & Memorizing Transformer & $1$ step
% \\
% & RMT & $t$ step
% \\
% & Longformer & $t$ step
% \\
% & StreamingLLM & $t$ step
% \\
% & Big Bird & $t$ step
% \\
% %% ************************************
\bottomrule
\end{tabular}
}
\vspace{-1.0em}
\end{table}

% 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

